Diffeomorphic interpolation for efficient persistence-based topological optimization

Topological Data Analysis (TDA) provides a pipeline to extract quantitative topological descriptors from structured objects. This enables the definition of topological loss functions, which assert to what extent a given object exhibits some topological properties. These losses can then be used to perform topological optimizationvia gradient descent routines. While theoretically sounded, topological optimization faces an important challenge: gradients tend to be extremely sparse, in the sense that the loss function typically depends on only very few coordinates of the input object, yielding dramatically slow optimization schemes in practice.Focusing on the central case of topological optimization for point clouds, we propose in this work to overcome this limitation using diffeomorphic interpolation, turning sparse gradients into smooth vector fields defined on the whole space, with quantifiable Lipschitz constants. In particular, we show that our approach combines efficiently with subsampling techniques routinely used in TDA, as the diffeomorphism derived from the gradient computed on a subsample can be used to update the coordinates of the full input object, allowing us to perform topological optimization on point clouds at an unprecedented scale. Finally, we also showcase the relevance of our approach for black-box autoencoder (AE) regularization, where we aim at enforcing topological priors on the latent spaces associated to fixed, pre-trained, black-box AE models, and where we show thatlearning a diffeomorphic flow can be done once and then re-applied to new data in linear time (while vanilla topological optimization has to be re-run from scratch). Moreover, reverting the flow allows us to generate data by sampling the topologically-optimized latent space directly, yielding better interpretability of the model.

==> defs.tex <==
% symbols =======================
% https://tex.stackexchange.com/questions/564216/newcommand-for-each-letter
\makeatletter
\newcommand\definealphabetloop[3]{%
  \ifx\relax#3\expandafter\@gobble\else\expandafter\@firstofone\fi
  {\expandafter\providecommand\expandafter*\csname#1#3\endcsname{#2{#3}}%
   \definealphabetloop{#1}{#2}}%
}%
\newcommand\definealphabet[2]{%
  \definealphabetloop{#1}{#2}abcdefghijklmnopqrstuvwxyzABCDEFGHIJKLMNOPQRSTUVWXYZ\relax
}%
\definealphabet{b}{\mathbb}%
\definealphabet{c}{\mathcal}%
\definealphabet{f}{\mathfrak}%
\definealphabet{r}{\mathrm}%
\definealphabet{s}{\mathscr}%
\definealphabet{t}{\mathtt}%
\definealphabet{B}{\mathbf}%
\makeatother

\newcommand{\bmu}{\bm{\mu}}
\newcommand{\btau}{\bm{\tau}}




\renewcommand{\epsilon}{\varepsilon}


%%% General maths notations
\newcommand{\dd}{\mathrm{d}}  % Integration
\newcommand{\prob}{\mathbb{P}}  % Proba of something
\newcommand{\perm}{\mathfrak{S}}  % Set of permutations
\newcommand{\diam}{\mathrm{diam}}  % Diam of a set
\newcommand{\supp}{\mathrm{spt}}
\newcommand{\mean}{\mathrm{mean}}
\newcommand{\diag}{\mathrm{diag}}  %TODO : c'est quoi ce truc ?
\newcommand{\dist}{\mathrm{dist}}
\newcommand{\linf}{\ell^\infty}
\newcommand{\Lip}{\mathrm{Lip}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\id}{\mathrm{id}}
\newcommand{\reshape}{\overrightarrow}
\newcommand{\card}{\mathrm{card}}
\newcommand{\vspan}{\mathrm{span}}
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\defeq}{\vcentcolon=}
\newcommand{\eqdef}{=\vcentcolon}
\newcommand{\Div}{\mathrm{Div}}
\renewcommand{\span}{\mathrm{span}}

\newcommand{\diffgrad}{\widetilde{\nabla}}

\newcommand{\p}[1]{\left(#1\right)}

%%% Mesure related notations
\newcommand{\cvvague}{\xrightarrow{v}}
\newcommand{\cvweak}{\xrightarrow{w}}
\newcommand{\cvu}{\xrightarrow{\|\cdot\|_\infty}}


%%% TDA related notations
\newcommand{\dgm}{\mathrm{Dgm}}
\newcommand{\Dgm}{\mathrm{Dgm}}
\newcommand{\Pers}{\mathrm{Pers}}  % persistence pour les diagrammes (ie distance au diagramme vide)
\newcommand{\pers}{\mathrm{pers}}  % persistence pour les points (ie distance à la diagonale)
\newcommand{\upperdiag}{\Omega} %{\R^2_>}  % The open upper half plane
\newcommand{\groundspace}{\overline{\upperdiag}}   % The closed upper half plane
\newcommand{\thediag}{{\partial \Omega}}  % Boundary of the half plane
\newcommand{\emptydgm}{\mathbf{0}}  %{\emptyset}
\newcommand{\Dp}{\OT_p}  % Wasserstein distance between PD in the Figalli and Gigli formalism
\newcommand{\Dinf}{\OT_\infty}  % W_infty distance between PD in the F&G formalism
\newcommand{\pdspace}{\DD}  % The space of persistence diagrams in its generality
\newcommand{\projop}{\mathbf{R}}
\newcommand{\projdiag}{\mathbf{p}_\thediag}
\newcommand{\gdist}{d}
\newcommand{\gcost}{c}
\newcommand{\pddist}{\mathbf{d}}
\newcommand{\dB}{\pddist_{\infty}}

%%% OT related notations
\newcommand{\round}{\mathcal{R}}
\newcommand{\pix}{\pi^{(1)}}  % first marginal of a transport plan \pi
\newcommand{\piy}{\pi^{(2)}}

\newcommand{\Adm}{\mathrm{Adm}}  % Set of admissible transport plans
\newcommand{\Opt}{\mathrm{Opt}}  % Set of optimal transport plans

\newcommand{\Smin}{\mathrm{Smin}}
\newcommand{\aprox}{\mathrm{aprox}}

\newcommand{\KL}{\mathrm{KL}}
\newcommand{\MMD}{\mathrm{MMD}}
\newcommand{\TV}{\mathrm{TV}}

\newcommand{\OT}{\mathrm{OT}}

\newcommand{\pioffdiag}{\pi^{\upperdiag \to \upperdiag}}
\newcommand{\pitodiag}{\pi^{\upperdiag \to \thediag}}
\newcommand{\pifromdiag}{\pi^{\thediag \to \upperdiag}}
\newcommand{\pidiagtodiag}{\pi^{\thediag \to \thediag}}

\newcommand{\pitrivial}{\pi_{\text{trivial}}}
\newcommand{\picross}{\pi_{\mu \otimes \nu}}


%%% Maths operators
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\minimize}{minimize}

%%% Useful additional shortcuts
\newcommand{\mtot}{{m_{\mathrm{tot}}}}
\newcommand{\Cp}{\mathcal{C}^0_{b,p}}
\newcommand{\gudhi}{\href{https://gudhi.inria.fr/}{\texttt{Gudhi}}}
\newcommand{\pot}{\href{https://pot.readthedocs.io/en/stable/}{\texttt{POT}~}}
\newcommand{\Cech}{\v Cech}
\newcommand{\PersLay}{\textsc{PersLay}}
\newcommand{\proj}{\mathrm{proj}}
\newcommand{\shift}{\mathrm{shift}}

\newcommand{\med}{\mathrm{med}}
\renewcommand{\div}{\mathrm{div}}

\newcommand{\exfig}{\includegraphics[scale=1]{example-image-a}}

%%% LaTeX shortcut
\newcommand{\emphindex}[1]{\emph{#1}\index{#1}}


%%% Misc
\newcommand{\todo}[1]{\textbf{\textcolor{red}{#1}}}

